Data-driven distributionally robust MPC for constrained stochastic systems

In this paper we introduce a novel approach to distributionally robust optimal control that supports online learning of the ambiguity set, while guaranteeing recursive feasibility. We introduce conic representable risk, which is useful to derive tractable reformulations of distributionally robust optimization problems. Specifically, to illustrate the techniques introduced, we utilize risk measures constructed based on data-driven ambiguity sets, constraining the second moment of the random disturbance. In the optimal control setting, such moment-based risk measures lead to tractable optimal controllers when combined with affine disturbance feedback. Assumptions on the constraints are given that guarantee recursive feasibility. The resulting control scheme acts as a robust controller when little data is available and converges to the certainty equivalent controller when a large sample count implies high confidence in the estimated second moment. This is illustrated in a numerical experiment.

==> arxiv.tex <==
\usepackage[pub=true]{arxivix}                            % pub=true for publication.

==> assets/hoeffding-offline-cost.tex <==
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:10,430.923696268764)
--(axis cs:10,428.373218130198)
--(axis cs:28,427.313323389506)
--(axis cs:81,426.413786584938)
--(axis cs:231,426.839926528798)
--(axis cs:658,424.646689146074)
--(axis cs:1874,405.155106356122)
--(axis cs:5337,392.148504620609)
--(axis cs:15199,382.136816958754)
--(axis cs:43288,375.680346720679)
--(axis cs:123285,370.949076059496)
--(axis cs:351119,367.818030523499)
--(axis cs:1000000,365.911290587564)
--(axis cs:1000000,369.273937723774)
--(axis cs:1000000,369.273937723774)
--(axis cs:351119,371.704285006003)
--(axis cs:123285,373.926349644618)
--(axis cs:43288,379.031676634325)
--(axis cs:15199,386.763582842576)
--(axis cs:5337,395.220164131795)
--(axis cs:1874,408.739421048849)
--(axis cs:658,428.212909260491)
--(axis cs:231,430.438118080173)
--(axis cs:81,429.088884750412)
--(axis cs:28,429.818717465107)
--(axis cs:10,430.923696268764)
--cycle;

\addplot [semithick, color0]
table {%
10 429.452860014795
28 428.654917088621
81 427.926608357137
231 428.315993561417
658 426.207807825095
1874 407.100578495845
5337 393.297693058116
15199 384.0533146323
43288 377.332447518329
123285 372.765769549288
351119 369.825271699884
1000000 367.537757996925
};

==> assets/hoeffding-offline-states.tex <==
\addplot [semithick, color0, opacity=0.1]
table {%
1.75 2
1.42537787568024 1.32488735769684
1.43112988356862 0.999203458849993
1.41742101887688 0.764135276982919
1.39740871821221 0.595998262400401
1.35456790996983 0.466674944812123
1.300193263088 0.365340186573028
1.22484132663981 0.283737839824368
1.13911609771224 0.21819730422075
1.05308239718203 0.167513123727803
0.963092530161865 0.128827851714436
0.873677896781508 0.097448810356701
0.791552948984564 0.0734611570911379
0.715601638050368 0.0531211826057261
0.646352512150394 0.0388391342179169
0.582276001843922 0.0276029432486071
};
% \addlegendentry{a}
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42359229140763 1.32513119237636
1.41677894250328 0.999178475870573
1.41181503297594 0.765081525685294
1.40302328240472 0.598625070579182
1.35638846146259 0.469602636335305
1.29423202743954 0.367693438934133
1.22288322384439 0.286878558419588
1.14501249676148 0.222839445719732
1.06180748442713 0.173395351116812
0.978858001800182 0.133077087821338
0.890276300013606 0.10195161987603
0.809614870777049 0.0758358269360812
0.744082146772743 0.0570366076491653
0.668386211589985 0.0433448942674101
0.60113492388354 0.0316075575366383
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42803198571261 1.32486621705919
1.4263761997967 0.995896979978726
1.40665904607471 0.762755654796974
1.39318558839798 0.597743529521714
1.34832354999029 0.469047802732962
1.28233527997606 0.365583688326933
1.21051524654231 0.285999275845745
1.12823774587073 0.220621953599806
1.04584428280512 0.169233176305299
0.968823232756275 0.128348391215913
0.881046343327951 0.0968274423610742
0.799995471190185 0.074480703930814
0.730639928412843 0.0551724941464786
0.654191578531653 0.0408365191560595
0.584318673182644 0.0273144569330158
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.41861834837393 1.32530836733062
1.42001826924092 0.998276848531454
1.41377479604539 0.765193232853749
1.40269967518884 0.59968047014755
1.35983084511432 0.469160473242747
1.30473444156282 0.366761786490893
1.23433342399456 0.283552178978079
1.15273807980602 0.218728308791907
1.06932033248664 0.168239884597694
0.988532550827246 0.128881815957981
0.90843838797114 0.0971645782818876
0.822320081510969 0.0723290369123858
0.745374172522144 0.0536950781900145
0.668442181276968 0.0384331484620618
0.599303072274955 0.027396229896674
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.43090896378439 1.32615327157227
1.42082691864113 0.995378702038387
1.41407018107811 0.762549618416476
1.39943929799491 0.596498589078392
1.36159725949021 0.46756586026825
1.29690206870973 0.363458999262806
1.21553848224 0.283152335057032
1.13000093988561 0.218680119264889
1.04458195029873 0.16830485348612
0.952208710051548 0.12888535294304
0.874650641854858 0.0978298429918193
0.795396602047098 0.0734610178786511
0.731372245879034 0.0546806770854399
0.657621094541591 0.0392095786658183
0.594556035207691 0.0274447717437947
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42449521329761 1.32436283855763
1.4263956590873 0.997102293057596
1.40747923566483 0.76182210505616
1.39638603198832 0.596208827164426
1.35469396139524 0.467731443023119
1.28871119410104 0.364241711307871
1.21443924985395 0.283325336609289
1.13477846213774 0.219037845696934
1.05160284046452 0.168524364987076
0.964582357707771 0.128022974118631
0.884303932638437 0.0961287812564575
0.799483205519106 0.0716760758486282
0.721394851093585 0.0538082475718445
0.655536356934393 0.0377493529846591
0.593820542342465 0.0252264445563171
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.415859258918 1.32455932933035
1.41631087383338 1.0000297987682
1.41277505179272 0.767326119825398
1.4029355788124 0.600857644025767
1.36202756047065 0.470493254035085
1.30049651860914 0.366762919137258
1.22592294530772 0.284013405186593
1.14681687960484 0.218858270170343
1.06685904865477 0.168209180884102
0.982019563102073 0.129039735597416
0.901928617456229 0.0962044106790821
0.820009777651226 0.0728775365481577
0.735003765317053 0.0541443033231612
0.664224631632099 0.037508342267666
0.592751801697803 0.02472259803857
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42415329350041 1.32423163244011
1.41567432779342 0.998346959227854
1.40737776308188 0.766017624943784
1.40209003426513 0.600290059345929
1.36302287335919 0.469988962104423
1.30685533995573 0.367318112252022
1.22262645219318 0.285711231285179
1.14211593598455 0.221293147019836
1.05604850891377 0.170670470666341
0.970235682499142 0.129115549456818
0.892540886528329 0.0981497339479268
0.808179276548939 0.0738936317308977
0.737215005300712 0.0546036987811363
0.670096253652441 0.0396008117542796
0.601338647858043 0.0266752299536549
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42034356669451 1.32427992693863
1.41088228230364 0.997784046932458
1.40525544066021 0.766158974516742
1.40030553622568 0.600746314675144
1.36630134439732 0.469355340160403
1.31070944896729 0.366742373402187
1.24029624774083 0.286149457173758
1.15407807768608 0.221057937875215
1.07711241545951 0.170731441141445
0.991190445573793 0.130741412186537
0.902076116021515 0.0987462408768096
0.827145727458648 0.075308291260184
0.74703040564108 0.0551475777973499
0.669881362041391 0.0398475528726317
0.605082109723343 0.027996655598325
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42983171181972 1.32648632745706
1.43084806739751 0.997542872295682
1.40990374626386 0.76196404513876
1.39373711026021 0.596258569738989
1.35203175298544 0.466612535015525
1.29286811657838 0.362906270180602
1.2185886034019 0.283661349112132
1.13685829172578 0.219144996175224
1.05970737509212 0.168083603330893
0.976178677700528 0.128566042315224
0.898113606847582 0.0971488630349241
0.814416619354259 0.0740543009647266
0.731970746172483 0.0539441452204497
0.671338762100117 0.0389707097966423
0.605285733840754 0.02555068373439
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42238090709422 1.32460558995538
1.42089364045462 0.998587092179416
1.41419401862769 0.765786598864063
1.39819135422227 0.598223803883672
1.35909755683502 0.468619116992894
1.29612539695466 0.365460530532772
1.21847450831369 0.283949999064409
1.1309847658817 0.220237245728517
1.04400001680443 0.169821960140306
0.954619502961177 0.12930996566161
0.873710265297148 0.0964088559799666
0.796424176753022 0.0718616509330411
0.713505270312786 0.0517175590110727
0.647386051793656 0.0382007013391709
0.582087824839825 0.0271952134616775
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42055824436537 1.32532663073431
1.4252192382279 1.00039619471208
1.41329044283357 0.767167452770685
1.40387289722544 0.599390728920517
1.35655339911023 0.468847288689158
1.30135349909283 0.365776196290175
1.22484292589936 0.285909612835221
1.14634246081472 0.221855781786141
1.06390276088817 0.171282010791816
0.979357372697397 0.129669644655955
0.894593737266988 0.0973359463913283
0.810029956301216 0.0716517427822771
0.736607434184524 0.0529131301181221
0.662998045612544 0.0375359439848929
0.596470425631494 0.0272990055701938
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42335144350768 1.32424670905189
1.42347239807298 0.998787762787968
1.40564855001881 0.763814937331701
1.38768045666223 0.599035148465828
1.34928096826151 0.471053982154531
1.2948011078814 0.367585696239746
1.22872058523368 0.286058583855542
1.14475770570137 0.222137876419922
1.05792990953431 0.170770920229333
0.980903303388299 0.130502098338129
0.893967368964696 0.0984721825712226
0.81945175116091 0.0732640702088093
0.741132050673939 0.0535544708382194
0.67032256031727 0.0382946834458896
0.595268018142866 0.0259125445213708
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.41602929194509 1.32537889151685
1.42266978780095 0.998293601203111
1.41463732216239 0.766498470774716
1.39970345584912 0.600672412689194
1.36253088064284 0.469485642248467
1.30191915164341 0.364794217559024
1.22591819100392 0.283845375121464
1.14899201502928 0.219741445038808
1.06835921123144 0.168049344841394
0.982579538187893 0.128436187999675
0.908349457485394 0.0970811233850183
0.824452336523096 0.072694591581463
0.742837747766816 0.0537920740162788
0.669134774753087 0.037066163186196
0.601695942296279 0.0255125600234919
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42302813184965 1.32424575958337
1.4293473132658 0.998540902676023
1.41531220924395 0.763180902269572
1.40460038215457 0.597689238550092
1.36549822850819 0.467790086020552
1.29561931060363 0.364896621774384
1.21989739538782 0.284323923235828
1.14511644211757 0.2194435822721
1.06357977240911 0.170662910754112
0.975954696639661 0.132181691805107
0.889604227294188 0.100304108796357
0.810722829909339 0.075291751759209
0.731446569501662 0.0551052495240801
0.657688897596379 0.0402634305006007
0.599196706601242 0.0278854349748046
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.41991593737142 1.32460282810298
1.41261597356719 0.998269136076111
1.40481260080684 0.766881088171177
1.39709969050728 0.600487980950645
1.35692676084282 0.470156905762262
1.2978980818167 0.365856611976252
1.22420384797758 0.284743105108414
1.13715734036884 0.221299665049574
1.05986058465556 0.16978443862191
0.974593620293093 0.128933808222702
0.895548563535978 0.096651144895573
0.814308984466823 0.0715107126869219
0.738400326338266 0.0508970040758902
0.673103271907399 0.0356186314244823
0.605570908431369 0.0244597641019316
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42995398174657 1.32640432022367
1.42064039426765 0.99596631495544
1.4052881662825 0.764566326488158
1.39112770613763 0.598255050804864
1.3528186577216 0.468145580722492
1.28621168637398 0.366562145869425
1.2211438099882 0.285262945665971
1.13998508751088 0.220593396357634
1.05867475862522 0.171319586216101
0.982976416630533 0.130767777767465
0.901427167172189 0.097762728957618
0.819322990514663 0.0723928301744903
0.737756763706552 0.0550566733408355
0.662699524316347 0.0393480005753141
0.598483388194834 0.0289537118549621
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42520718598056 1.32664227264572
1.4268873652652 0.999820639340756
1.41115541258457 0.76596653733138
1.3978166757525 0.600890169501917
1.367519249207 0.470023323002893
1.30424938270715 0.365909068147462
1.22978151966465 0.284091808647669
1.15068269837236 0.219760603574593
1.06446677502363 0.170227179084553
0.975319901695415 0.13058673597729
0.890975878343665 0.0997439214158399
0.818828252944445 0.0745294740884314
0.744947030955192 0.0552476441120482
0.669115801795831 0.0402444313551126
0.604002328689032 0.0287602250422201
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42627387967934 1.32339762092443
1.42475491883221 0.996492353462939
1.41837679538624 0.763755209779994
1.40054166367851 0.596576117481386
1.36770258670283 0.46613794885913
1.30049118192366 0.36260494648016
1.23208392434309 0.281332229348745
1.14666039377436 0.217846942468265
1.06126614989338 0.16696802379162
0.980297580496914 0.128636976275222
0.902024187869935 0.0982276920013228
0.823515503807489 0.071823799935413
0.754781533435238 0.0532143121534531
0.684587538442749 0.0394866689368803
0.623419539086425 0.028121062253896
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42657005598462 1.32548964232099
1.4186345979439 0.996352238295665
1.41002084410434 0.762792779424877
1.39569823004226 0.598014598969967
1.35811397484626 0.467037053596473
1.2930162992708 0.364761755897012
1.21820381807328 0.283264392710467
1.14135148062723 0.218289544181389
1.05562833361934 0.167211685753083
0.966350685723587 0.126941518316666
0.887700841711866 0.0962098400681014
0.803926670419619 0.0718116444516356
0.720722739479058 0.0522262246270669
0.661656049418071 0.0375969689955726
0.599057081642757 0.0262065611874269
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.4288013189938 1.32617935849453
1.41951837209837 0.9970588763639
1.41546233309616 0.765046406041165
1.40490290750034 0.598583828670273
1.36197675913156 0.466514624811623
1.29493751732191 0.364051521580815
1.22597667857928 0.283572306918978
1.1447097827768 0.219214834239588
1.06191679593808 0.168824641786687
0.984497985441996 0.129198760782671
0.893551023963628 0.0966211078512466
0.821223428641677 0.0711804702292192
0.748089514933949 0.0521409273708804
0.674515415973218 0.037406338377936
0.612969797018679 0.0258910939587545
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42892993078776 1.32490784302394
1.43371313700191 0.996643151547978
1.41991029313088 0.761628747473988
1.40051135046408 0.596992195971227
1.3685741875276 0.467174086913766
1.30518869340962 0.364153991389931
1.2215592053528 0.282905576204613
1.14253277950883 0.220025913324043
1.06381366709937 0.168968603662234
0.977812586135936 0.130284128229363
0.894311472411249 0.0982625924079336
0.821574540378918 0.0746872118334157
0.745320675575246 0.0545920859732865
0.66328007640034 0.0400795987762963
0.592825851133928 0.0262708026274582
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.43395276806119 1.32464658443341
1.42417503224816 0.995236355897048
1.4146349233032 0.762132539952572
1.39537880484036 0.59678921278014
1.35974556216943 0.467586121975799
1.29494483619808 0.366579434266473
1.2150964318714 0.283462402716381
1.14041022325572 0.219659846604661
1.05432349147811 0.168014213535447
0.973208447182364 0.128750984070969
0.89295323749095 0.0981115809292859
0.817031691402998 0.0731587130559238
0.739460972467527 0.0522654063990817
0.663769848692918 0.0379351450281296
0.602576041428854 0.0271326714099241
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.4299098501455 1.32554607295422
1.42096142372743 0.995590985663094
1.41414647327144 0.762708548207264
1.39930860141759 0.598512658298034
1.36094084927791 0.467622327209719
1.30075497671094 0.363935437299848
1.23502050587932 0.282342435390155
1.15428167259918 0.21881086913425
1.07011138098825 0.1664398710924
0.97712289054843 0.126682935978572
0.895496139723393 0.0957844655022887
0.81042914494035 0.0703348798100062
0.732451705721737 0.0513025713212839
0.663790729937809 0.0365954877128813
0.600136925333656 0.0248780566830375
};
\addplot [semithick, color0, opacity=0.1, forget plot]
table {%
1.75 2
1.42560011713486 1.32517170357733
1.42049996901639 0.997058860324533
1.40389833227539 0.76588718541421
1.38552610148758 0.60090705930642
1.34420009449138 0.469554482725192
1.2884110688056 0.365816139996802
1.21921994605021 0.284142330998182
1.14184203117055 0.219002424257206
1.06238510180637 0.169074928894186
0.985933433223196 0.129056366697572
0.900153412104234 0.0973733379930692
0.81052200028163 0.0722325375457782
0.736125761096836 0.0547997992046643
0.661291487489284 0.0405629970011394
0.589355519017378 0.0280358513678559
};
\addplot [semithick, color1, opacity=0.1]
table {%
1.75 2
1.48386472081715 1.35184812654439
1.47875148689332 1.01634410755729
1.47517898574642 0.783389820711331
1.45954025987943 0.615537397031214
1.41595940651877 0.483518953266124
1.35720073450481 0.377937657608974
1.28539379144827 0.294798370806165
1.21111972581531 0.229344458770719
1.12020385021378 0.176923334727717
1.03479934743708 0.135209455640501
0.956622165302073 0.104255456876169
0.867087467877521 0.0795191254623893
0.794176822860735 0.0600597432243394
0.7289362612094 0.0444526053645821
0.652253217330285 0.0325205474855044
};
% \addlegendentry{b}
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47021881233452 1.35037665104904
1.47062025679235 1.02200622923947
1.47644927642082 0.792004285649383
1.46829178160318 0.622122344586515
1.42469688434866 0.489195819430315
1.36204407206379 0.383810652605152
1.28194280196713 0.299737840019788
1.19754424985937 0.232491232320897
1.11324976942178 0.180072684732986
1.02460157577013 0.138741186465887
0.947102886236004 0.108179739410615
0.859419996764554 0.0819504740536981
0.790373305850098 0.0633113031079025
0.725534383031545 0.0479419801157277
0.662889578399287 0.0364855729989363
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.48217474841708 1.35001684660644
1.48292048976118 1.01568825776452
1.47351474300053 0.782157973527915
1.46655195464822 0.615101974289989
1.43087374434367 0.482164778923175
1.36452225259268 0.377055957500945
1.28559500587664 0.296589010905638
1.21068640803987 0.231569909930127
1.12401316533767 0.17973260494046
1.0327882550164 0.140113895312351
0.952676943105363 0.108757830266629
0.877793331888733 0.0818325321824743
0.791862705626896 0.0622221790951659
0.719063413260493 0.0456039721433689
0.654702081465351 0.0341859451387765
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47646489134302 1.35027696059401
1.47587905164109 1.01870004536271
1.47577045721252 0.787693054633419
1.46418011969885 0.61811584261703
1.43131030742009 0.483909456222433
1.36033477799169 0.378621263933949
1.29112197702128 0.296504619430418
1.20816629388088 0.229572670965404
1.12083399108362 0.178940292868205
1.03538069188935 0.138189461585052
0.953598480515978 0.106893012277354
0.863818593888378 0.0808691214456094
0.784653132284885 0.0614005674217252
0.712177252977913 0.0482773272049423
0.640340535256511 0.0365935067796568
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47092099031288 1.35003532169345
1.47652666785311 1.02131132783098
1.48064926979574 0.789126590947351
1.46882637609721 0.62078566124471
1.42725374491977 0.486357878804893
1.36870055313059 0.381087978797109
1.30353956070353 0.297048867389002
1.22632817413588 0.231701606134034
1.14402501873273 0.180042586919604
1.05330841811356 0.138607368749783
0.965914944793343 0.106254329890618
0.880902290034343 0.0816563833910196
0.807582335418587 0.0611088702248509
0.736368335093068 0.0445315800880631
0.665519257419752 0.0332524119606114
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47748813725073 1.35091868628286
1.47766328585882 1.01847532217632
1.47344566572875 0.785518860980297
1.45771058119424 0.619360511797188
1.4140488456597 0.485587844149191
1.35634003887331 0.379686693417468
1.2755316069582 0.295970477638156
1.19347871874453 0.230421828434979
1.11116482719294 0.17863119910298
1.02043445488553 0.138627113421832
0.936379595745293 0.106298360844437
0.849109743885833 0.0804089881808325
0.775490262510059 0.0621007760672497
0.704844465194687 0.0475813067096008
0.636052655664309 0.0354303643864342
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47581633201447 1.34995964463358
1.47745503928714 1.01849599998687
1.47306859142125 0.787657638851783
1.46527713537068 0.619024867740234
1.42338217919989 0.486842948511921
1.36533159621037 0.38146300223484
1.28928270295981 0.296749594647265
1.2103157471446 0.229860899924136
1.12487644684843 0.179123501048385
1.04058890027242 0.13973651872568
0.961952739504802 0.106816028132269
0.877082427546814 0.0816560180272263
0.804253371017296 0.0605777676803066
0.721902215082467 0.0440812935941127
0.646940189433192 0.0308992364235975
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.48361857362031 1.35124156805069
1.4739070506378 1.01521337513313
1.47319669302232 0.786009626979122
1.46135356822005 0.618696063885097
1.42023149130186 0.486962948565199
1.35878117432003 0.380236018812402
1.28947973718894 0.295985420900815
1.20826785506496 0.229471306976232
1.12994954994289 0.178486323168335
1.0373153852446 0.137580397587811
0.947856074880606 0.105469683329456
0.862013397087098 0.0791900980978808
0.780306092840726 0.0593917586991512
0.708616005871632 0.0430889589006168
0.646807784532372 0.0305400435119394
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47283879857654 1.34915481759684
1.474374738452 1.01846781913806
1.47144311657862 0.78578478785422
1.4576968056606 0.618717002735026
1.41646030632123 0.485344303579319
1.35679401591529 0.380265850730744
1.28328813399197 0.297773500605997
1.20089804025106 0.231468360140791
1.11534338982875 0.178706108007739
1.03170545172026 0.138983685981259
0.948284373691027 0.108914586244132
0.874258319137392 0.0831348247433276
0.794926753489809 0.0641353809356495
0.720506846330578 0.0489576287768927
0.648472274861484 0.0362268225631552
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47863220180574 1.3503227870035
1.47368174679461 1.01831390028276
1.47578677176508 0.787392300939195
1.46255185816092 0.61957660254688
1.42137304649196 0.485716960270235
1.36638031248239 0.379449374693594
1.29521249994684 0.296167085173109
1.21930114230488 0.230736447693551
1.12990272661839 0.18038713643653
1.04777775085962 0.141357189416948
0.961630497706544 0.108655771242933
0.88608949212053 0.0826428959004721
0.809923223345984 0.0643249560936387
0.7439765746161 0.0474914035036281
0.672186557823129 0.0356501306991403
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47313030999183 1.35220955937201
1.47148412076128 1.01984883360187
1.47393426317349 0.78983152929109
1.46696330880665 0.621380549212692
1.419195152863 0.487818263444034
1.35902449883728 0.381497082705543
1.28008168160533 0.298503636411446
1.20342689791166 0.232965461040021
1.11755311253242 0.181984407341155
1.03183877576243 0.14104332587369
0.94125491269761 0.108123614465084
0.854644180826042 0.0827384135033273
0.788064030047003 0.0632474167188947
0.719827205602346 0.046160187119261
0.653203605831223 0.0323717617126147
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47456447149962 1.35043986647155
1.4794012407342 1.02052013562574
1.4782470480592 0.787476267418634
1.46110882427338 0.618421177846718
1.41567018015368 0.484013816529614
1.34877132304255 0.3780723009223
1.27730079307856 0.296146364598427
1.19805011428377 0.230627114815571
1.11308982506658 0.178530463116232
1.02593356023411 0.137961797497203
0.950340249854789 0.105468779561621
0.859966687426422 0.0795896604403501
0.786676579098676 0.0597776435334279
0.720722778566108 0.045321187217635
0.651147372150231 0.0326849561676914
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47088167149114 1.35154775539514
1.48460847706707 1.02216043590536
1.47654817632792 0.78493735381461
1.46207158225489 0.617843063005869
1.42274894868438 0.483544706596712
1.35950174829738 0.379575193873234
1.2807286975741 0.29753418050314
1.19217312006508 0.232092564918884
1.11050786669981 0.179590159834718
1.03024799900841 0.138104915561619
0.945362721084157 0.106485342315449
0.865176888159786 0.0807305071996694
0.785269164651415 0.0608057693754717
0.711469188818961 0.0448972261270358
0.644277578175127 0.0323655827784652
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47504841554655 1.35014952543755
1.47027209165551 1.0193685749689
1.47676878564277 0.790079578064116
1.47013251805191 0.621621136244576
1.43297102012228 0.488024353159247
1.37475988528207 0.383597358306066
1.3030151729587 0.300747751012077
1.22613026610266 0.23442139828948
1.14077294691248 0.180836245398101
1.05162009202958 0.139851097610451
0.961069487927081 0.10778938869468
0.876404958484462 0.0837706417848136
0.797879336835388 0.0643594820764921
0.722853997519998 0.0483217929609689
0.66121571416611 0.0348973555236318
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.4797083572561 1.34989474705218
1.47330833223232 1.01737023376169
1.48511146437432 0.787553572881948
1.47516569824837 0.619652221849639
1.43471850442986 0.487045283112067
1.37809345474799 0.381197580491341
1.30385255623482 0.297899502507385
1.2178714843589 0.231402262233031
1.13237676717795 0.178644705023335
1.05222470475725 0.13728331054273
0.970474627077698 0.106187930235701
0.889674272787066 0.0810090614415478
0.808822996521759 0.0622312838060057
0.736288805012001 0.0482345368562798
0.668007539340269 0.037581293535188
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47043421431027 1.34914588338136
1.47127194025872 1.02132068203485
1.48081822872606 0.79012583207724
1.4667668329424 0.621571122602728
1.42629024917524 0.487427135306085
1.3675320563006 0.382085821212125
1.29726110586143 0.297392624843274
1.21905733254856 0.23248004028544
1.13348567818335 0.182077065190702
1.04876311111394 0.139096374755513
0.959817857582513 0.10732532769419
0.867040763926316 0.0819544115906233
0.790582203894767 0.0622868318354868
0.719401881156844 0.0464650069652196
0.648514459103891 0.0326869276264309
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47495007201533 1.34862176897783
1.47173547830004 1.01826661632716
1.47301921763951 0.789703373007052
1.45983857500828 0.62046658571406
1.41207071599977 0.487556742879151
1.35790158129646 0.381889761377746
1.28155840169717 0.296796065554996
1.19680500772278 0.230554304195008
1.11513297418768 0.179565434804953
1.02572764113994 0.140485924735065
0.940134662071143 0.109214737120487
0.861559320996595 0.0829878189087776
0.779952478557054 0.0636926670374866
0.717086145453135 0.0489431627481082
0.653007210245288 0.037318030284588
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47778563297519 1.34950614596927
1.47512408951397 1.017962968502
1.47806076035399 0.788332089954656
1.47305336364187 0.620100961795836
1.43107700528588 0.487020225816464
1.36436377199206 0.381418538207112
1.2828116422694 0.297763958323372
1.20115870439122 0.233128823224243
1.11296221916889 0.181752391495946
1.02752450473388 0.139860053516804
0.943818096816204 0.106907447747187
0.866472577688926 0.0821553452709989
0.793667648147501 0.0617111993267316
0.720849463469903 0.0480322254986696
0.661944322801912 0.0355440159018437
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47619350856417 1.34983595366926
1.47198640597012 1.01831778618361
1.48483866660139 0.787795498566749
1.47601367582082 0.621472298842817
1.43963307198399 0.486744044789123
1.36890406901708 0.381067709684372
1.29675997990554 0.29779045272955
1.21147584008288 0.231749762231476
1.12514844555967 0.179360980901158
1.04534919992712 0.139677208005262
0.955114875130265 0.107700862603873
0.872907646337662 0.0826159433401992
0.790996482247774 0.0642378512124466
0.713586127905816 0.0490420264397889
0.651743679691651 0.0361167829204473
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47568111279627 1.35203710129575
1.48390931162782 1.02129286235493
1.46866502104553 0.785150928440402
1.46440688877064 0.617476722033345
1.42189956553852 0.484100581202894
1.35869525372206 0.3785648865761
1.27932125545662 0.295668429613689
1.19351486533013 0.230419592697967
1.10461220272632 0.177899362791384
1.01553548328992 0.136294832933985
0.924929706281644 0.106215472646863
0.850176813905485 0.0815547199109476
0.781129987387928 0.0628160308221532
0.711219495846551 0.0459540576476338
0.636725331556408 0.0334080356917192
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.475589937582 1.35040676697823
1.47631043549144 1.01883769132696
1.48083964756928 0.785772680825414
1.47791504449532 0.6177555122957
1.4287188552547 0.485219548870537
1.37554227952014 0.379478196299001
1.30771600343972 0.295919222991869
1.22159874924194 0.231550045085513
1.13470026587993 0.179680475957295
1.05043060157424 0.138459313843909
0.958497348797202 0.107639781265012
0.880520351067908 0.0810608041736118
0.796414055706679 0.0625509165567817
0.719459594425836 0.0476403680859038
0.651315862918947 0.0356140298931319
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47865111310456 1.35125435351555
1.47619273319231 1.01858215502154
1.47186182967456 0.785117166820109
1.46110328333727 0.618036128547981
1.42287095472836 0.484356824387079
1.35399002975954 0.380235401349771
1.27579612941029 0.297254482101685
1.19562761493694 0.232853493761172
1.11114589830847 0.182109577347793
1.0267122663393 0.141604949081073
0.939359401348322 0.109309452931389
0.858836248918091 0.0819495468959828
0.791532558892522 0.0618808178507005
0.720288182763099 0.0466461541172636
0.651781903996702 0.034811971691118
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.48390436071833 1.35090875089948
1.46694343823769 1.01707178300876
1.47340936038028 0.78920346618295
1.46640028173643 0.620669935507223
1.42724596780819 0.486488285654379
1.36890415469815 0.380532095634881
1.28680896462013 0.297409815501349
1.19737203795051 0.23209578529208
1.11084034785793 0.180433806518747
1.02363778670646 0.139109166858487
0.943799901513612 0.108063475006316
0.858265260714536 0.081762646908927
0.790122498947924 0.061671735589079
0.719833467506061 0.0456654598467119
0.6455002872691 0.0328897549713526
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.4821663630028 1.35027465173732
1.46984204132049 1.01650555013787
1.48141343756769 0.788641489135026
1.46722107834426 0.622399907356883
1.42010029725623 0.487055139534254
1.34972457303461 0.381196417213337
1.27669237799435 0.298646013546167
1.19397420942513 0.232067509320841
1.10920503964962 0.179970717349973
1.02271436414826 0.138823464500174
0.948472911472365 0.107056944412612
0.866982106501946 0.0837258652987447
0.794700760659571 0.0642540284076912
0.725784076897568 0.048003839844119
0.657789296160295 0.0356472230186874
};
\addplot [semithick, color1, opacity=0.1, forget plot]
table {%
1.75 2
1.47106561577748 1.35247507188069
1.48290784524261 1.02391880106859
1.47877258644446 0.787529792666897
1.47687549205278 0.61892458085249
1.44268745367751 0.486539896565621
1.37883430695055 0.380073638793491
1.29951187633794 0.297697553974356
1.21835708042472 0.231568361613203
1.12941004791211 0.17986489363992
1.04525861217177 0.139295951747793
0.963635557072081 0.107002441477651
0.870465028313443 0.0815383629586099
0.796619110554234 0.0621723259940499
0.723646635475752 0.047627875563824
0.665139785991213 0.0354625608086827
};
\addplot [semithick, white!50.1960784313725!black, dashed, forget plot]
table {%
1.5 0
1.5 2
};
